Assessing the Real-World Impact of Post-Quantum Cryptography on WPA-Enterprise Networks

The advent of large-scale quantum computers poses a significant threat to contemporary network security protocols, including Wi-Fi Protected Access (WPA)-Enterprise authentication. To mitigate this threat, the adoption of Post-Quantum Cryptography (PQC) is critical. In this work, we investigate the performance impact of PQC algorithms on WPA-Enterprise-based authentication. To this end, we conduct an experimental evaluation of authentication latency using a testbed built with the open-source tools FreeRADIUS and hostapd, measuring the time spent at the client, access point, and RADIUS server. We evaluate multiple combinations of PQC algorithms and analyze their performance overhead in comparison to currently deployed cryptographic schemes. Beyond performance, we assess the security implications of these algorithm choices by relating authentication mechanisms to the quantum effort required for their exploitation. This perspective enables a systematic categorization of PQ-relevant weaknesses in WPA-Enterprise according to their practical urgency. The evaluation results show that, although PQC introduces additional authentication latency, combinations such as ML-DSA-65 and Falcon-1024 used in conjunction with ML-KEM provide a favorable trade-off between security and performance. Furthermore, we demonstrate that the resulting overhead can be effectively mitigated through session resumption. Overall, this work presents a first real-world performance evaluation of PQC-enabled WPA-Enterprise authentication and demonstrates its practical feasibility for enterprise Wi-Fi deployments.

==> prelude/configurables/authors.tex <==
%\author{LLLukas Popperl\IEEEauthorrefmark{1}\orchid{0000-0003-3620-2336}, Nils Lohmiller\IEEEauthorrefmark{1}\orchid{0009-0008-1301-4002}, Tobias Heer\IEEEauthorrefmark{1}\orchid{0000-0003-3119-252X}}

%\affil{University of Applied Sciences Esslingen, Germany}
%\corresp{CORRESPONDING AUTHOR: First A. Author (e-mail: author@ boulder.nist.gov).}
%\authornote{This work was supported by the Natural Sciences and Engineering Research Council (NSERC) of Canada.}
%\markboth{Preparation of Papers for IEEE OPEN JOURNALS}{Author \textit{et al.}}









==> prelude/configurables/thanks.tex <==
\thanks{
    This work has been funded by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) – Project-ID 528745080 - FIP 68. %Additionally, this research was supported by the project "FHP:
    %Qualifizierung und Entwicklung des professoralen Personals der Hochschule Esslingen für zukunftsweisende Themen" (FKZ: 03FHP115) as part of the Federal States Program "FH-Personal", funded by the BMBF and MWK Baden-Württemberg.
    The authors alone are responsible for the content of the paper.
}
